Max-Information, Differential Privacy, and Post-Selection Hypothesis Testing

In this paper, we initiate a principled study of how the generalization properties of approximate differential privacy can be used to perform adaptive hypothesis testing, while giving statistically valid $p$-value corrections. We do this by observing that the guarantees of algorithms with bounded approximate max-information are sufficient to correct the $p$-values of adaptively chosen hypotheses, and then by proving that algorithms that satisfy $(\epsilon,\delta)$-differential privacy have bounded approximate max information when their inputs are drawn from a product distribution. This substantially extends the known connection between differential privacy and max-information, which previously was only known to hold for (pure) $(\epsilon,0)$-differential privacy. It also extends our understanding of max-information as a partially unifying measure controlling the generalization properties of adaptive data analyses. We also show a lower bound, proving that (despite the strong composition properties of max-information), when data is drawn from a product distribution, $(\epsilon,\delta)$-differentially private algorithms can come first in a composition with other algorithms satisfying max-information bounds, but not necessarily second if the composition is required to itself satisfy a nontrivial max-information bound. This, in particular, implies that the connection between $(\epsilon,\delta)$-differential privacy and max-information holds only for inputs drawn from product distributions, unlike the connection between $(\epsilon,0)$-differential privacy and max-information.

==> prelims_linear_codes.tex <==
\subsection{Preliminaries for Linear Codes}

For the current and the next section, we limit our scope to $\mathbb{F}_2$, i.e., the finite field with 2 elements. First, we will define linear codes as we will use them extensively in the proof of the theorem in the next section.

\begin{defn}[Linear Code] 
A code $C \subseteq \{ 0,1 \}^n$ of length $n$ and rank $k$ is called linear  iff it is a linear subspace of the $k$-dimensional vector space $ \mathbb{F}^n_2$. The vectors in $C$ are called codewords. 
\end{defn}
The minimum distance $t$ of a linear code $C$ is $t = \min\limits_{c_1, c_2 \in C} dist_{Hamm}(c_1,c_2),$ where, $dist_{Hamm}(p,q)$ denotes the Hamming distance between binary vectors $p$ and $q$.

We now define parity check matrices, which can be used to construct linear codes. Every linear code has a parity-check matrix corresponding to it. Thus, given a parity-check matrix, one can reconstruct the corresponding linear code.
\begin{defn}[Parity-check matrix]
For a linear code $C \subseteq \{ 0,1 \}^n$ of length $n$ and rank $k$, $H\in \{ 0,1 \}^{(n-k)\times n} $ is a parity-check matrix of $C$ iff $H$ is a matrix whose null space is $C$, i.e., $c \in C$ iff $Hc = \textbf{0}$, where $\textbf{0}$ represents the zero vector. 
%The minimum distance of the code is the minimum number $t$ such that every $t$ columns of $H$ are linearly independent while there exist $t+1$ columns of $H$ that are linearly dependent. 
\end{defn}

%\omnote{the following theorem proves that there exists a linear code for the parameter values we have chosen, and the theorem follows from 1) the Gilbert-Varshamov bound (cited from book of Lint), and 2) $h_2(x) \leq cx\ln(\frac{1}{x})$ for $x \in (0,\frac{1}{2})$ and $ c \geq 3$. Can show proof if required.}
Now, we state a theorem which shows the existence of high-rank linear codes when the minimum distance is less than half the code length. 

\begin{theorem}[From Theorem 5.1.8 in \cite{L99}]
For every $t \in (0,\frac{n}{2})$, there exists a linear code of rank $k$ such that $k \geq n - 3t\ln (n)$. 
\label{thm: existence}
\end{theorem}

\begin{comment}
A linear code $C\subseteq \{ 0,1 \}^n$ with minimum distance $t$ and rank $k$ has exactly $2^k$ codewords. Also let $R = \dfrac{k}{n}$ denote the rate of the code, and $C$ as $\delta = \dfrac{t}{n}$ denote its relative distance. We know that:


\begin{theorem}[Gilbert-Varshamov bound]
There exists a linear code $C\subseteq \{ 0,1 \}^n$ with rate $R$ and relative distance $\delta$ if
\begin{enumerate}
\item $\delta < \dfrac{1}{2}$, and
\item $R \leq 1 - h_2(\delta)$, where $h_2(x)$ is the binary entropy function \rynote{Can we use another variable, because $H$ is already the  parity check matrix.}\omnote{Good catch! Does $h_2$ seem good?}\omnote{There is probably another way we can show the existence of codes for our chosen parameters (without using $R, \delta$ and $h_2$!). Will verify and add soon.}\rynote{I guess $H$ is more commonly used for entropy.  Can we change the matrix variable name?}\rynote{Actually, why even have this notation here?  Do we ever need the entropy function again?} defined as $h_2(x) = - x log_2(x) - (1-x) log_2(1-x)$.
\end{enumerate}
\end{theorem}
\end{comment}

Next, we will define an affine code, which is a translation of a linear code by a fixed vector in the vector space of the linear code. 

\begin{defn}[Affine Code]
Let $C \subseteq \{ 0,1 \}^n$ be a linear code of length $n$, rank $k$ and minimum distance $t$. For any vector $b \in  \mathbb{F}^n_2$, the code defined by $C_a = \{ c + b : c \in C \}$, where $a = Hb$, is called an affine code.
\end{defn}

\begin{lemma}
If $C$ is a linear code with parity check matrix $H$ and minimum distance $t$, then the affine code $C_a$ also has minimum distance $t$.  Further, for all $c' \in C_a$, we have $H c' = a$.  
\label{lem:codes}
\end{lemma}
\begin{proof}
Let $c' \in C_a$.  We know that there exists a $c \in C$ such that
\begin{align*}
Hc' & = H(c+b) = \textbf{0} + Hb = a.
\end{align*}
\end{proof}

Lastly,  we define the concept of a Hamming ball around a point, which is helpful in understanding the point's neighborhood, that is, the points close to it when the metric of measurement is Hamming distance.

\begin{defn}[Hamming ball]
A Hamming ball of radius $r$ around a point $p \in \{0,1\}^n$, denoted by $B_r(p)$, is the set of strings $x \in \{0,1\}^n$ such that $dist_{Hamm}(x,p) \leq r$.
\end{defn}

As $B_r(p)$ includes all the strings in $\{0,1\}^n$ which are at a distance of at most $r$ from $p$, we define the volume of such a ball, denoted by $Vol(B_r)$, as: $$Vol(B_r) \stackrel{def}{=} \left |B_r(p) \right | = \sum\limits_{i=0}^{r} | \{ x \in \{ 0,1 \}^n : dist_{Hamm}(x,p) = i \} | =  \sum\limits_{i=0}^{r} {n \choose i}.$$ Note that $Vol(B_r)$ is independent of the point around which the ball is centered.

\begin{comment}
Let the elements of a code $C \subseteq \{ 0,1 \}^n$ with minimum distance $t$ be called `stable' instances. So, around every codeword in $C$, there is a unique ball of radius $\frac{t-1}{2}$ in which no other codeword of $C$ is present. Define $\cK_{dist}$ to be an algorithm such  that on input $D$ and parameters $\eps, \delta > 0$, $\cK_{dist}$ computes the distance $d$ from $D$ to the nearest stable instance, and adds Lap$(1/\eps)$ noise to get an estimate $\hat{d}$ of $d$. Finally, if $\hat{d} < \frac{t-1}{2} - \frac{\log (1/\delta)}{\eps}$, then it releases the nearest stable instance, otherwise it outputs a special symbol $\bot$. We can now make use of the following:

\begin{proposition}[Part of Proposition 3 in \cite{ST13}]
$\cK_{dist}$ is $(\eps, \delta)$-differentially private.
\label{prop: alg_eps_delta}
\end{proposition}



We state some properties of linear codes which we will use in this paper.  For a linear code $C$ of length $n$,
\begin{enumerate}
\item the vector $\vec{0}$ is always a codeword of $C$.
\item the minimum distance of $C$, denoted by $t$, can be defined as $$t = \min\limits_{\vec{x} \in C, \vec{x} \neq 0} w_{Hamm} (\vec{x}),$$ where $w_Hamm(\vec{y})$ denotes the Hamming weight of $\vec{y}$.
\end{enumerate}

\end{comment}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> pvalues.tex <==
\section{Adjusting p-values for Multiple Hypothesis Testing}


Let $\cX = \{0,1 \}^d$.  We want to test pairwise independence for all pairs of the $d$ variables.  We will assume the null hypothesis holds where all the variables are independent, i.e. $\cD$ is some Bernoulli distribution and $\cP = \cD^d$.  We then sample dataset $\bX \sim \cP^n$.  Consider the bad data analyst that wishes to report something significant, so he conducts all $m = O(d^2)$ possible pairwise independence tests and takes the test with the smallest p-value.  Let $\phi_i: \cX^n \to [0,1]$ be the p-value attributed to the hypothesis test with index $i \in [m]$.  We know the following
$$
\prob{\phi_i(\bX) \leq \gamma} = \gamma.
$$ 

We want the probability that the data analyst falsely rejects that some pair of variables were not independent to be at most $\alpha$ (i.e. significance $1-\alpha$).  Thus we have we need to select a $\gamma$ such that 
$$
\prob{\min_i\{\phi_i(\bX) \} \leq \gamma} = 1- (1-\gamma)^m \leq \alpha.
$$

Now, imagine that each each hypothesis test is $\epsilon$-differentially private and has p-value $\tilde \phi_i: \cX^n \to [0,1]$ where
$$
\prob{\tilde \phi_i(\bX) \leq \gamma} = \gamma.
$$

Consider the algorithm $\cA: \cX^n \to (\cX^n \to [0,1])$ where
$$
\cA(\bX) = \tilde\phi_{ \arg\min_{i \in [m]}\{ \tilde\phi_i(\bX)\} }.
$$

Note that from post-processing and from \cite{DRV10}, we know that $\cA$ is $(\epsilon\sqrt{8m\log{1/\delta}} , \delta)$-differentially private.  We can use \Cref{thm:main} to conclude that if we want our analyst to falsely reject any independence test with probability at most $\alpha$, we require to set $\gamma$ such that 
$$
\prob{ \phi(\bX) \leq \gamma \quad \& \quad \cA(\bX) = \tilde\phi} \leq \gamma 2^k + \beta \leq \alpha.
$$
where 
$$
k = O \left( \epsilon^2n+ n \sqrt{\delta \epsilon} (m \log(1/\delta))^{1/4}\right) \qquad \beta = O\left(  n \sqrt{\delta/\eps} (m \log(1/\delta))^{-1/4} \right) .
$$

Which then simplifies for $\epsilon = \Theta(1/\sqrt{n})$ and $\delta = e^{-O(n)}$ to setting $\gamma$ such that 
$$
\gamma 2^{O\left( \sqrt{nm} \exp[-n/2] \right)} + \frac{n\exp[-n]}{\sqrt{m}}\leq \alpha
$$
\rynote{Need to figure out constants}
$$
\implies \gamma \leq \frac{\alpha - \frac{n \exp[-n/2]}{\sqrt{m}}}{\exp[\sqrt{nm} \exp[-n/2]]}
$$
as opposed to before we would need 
$$
\gamma \leq 1- (1-\alpha)^{1/m}
$$

\iffalse
Consider a data analyst that wants to run multiple hypothesis tests adaptively at some significance level $1-\alpha$ on a single dataset.  Let $\cA: \cX^n \to \cH$ have outcome space the set of all hypothesis tests $\cH$ with significance $1-\alpha$ and $\cI_\infty^\beta(\cA,n) \leq k$.  We will denote the set $\cO_\alpha$ as the set of outcomes where an analyst would reject the null hypothesis at significance $1-\alpha$,
$$
\cO_\alpha = \{(\bbx, h): h(\bbx) \leq \alpha \}.
$$
We will denote the random variable $H = \cA(\bX)$.  We then have
\begin{align*}
\prob{H(\bX) \leq \alpha}  = \prob{(\bX,H) \in \cO_\alpha} \leq 2^k \alpha + \beta.
\end{align*}

Consider a sequence $\cA_1, \cdots, \cA_m$ with ranges that are $1-\alpha$ significant hypothesis tests $\cH_1, \cdots, \cH_m$ such that for each $i \in [m]$, $\cA_i: \cX^n \times \cH_1 \times \cdots \times \cH_{i-1} \to \cH_i$ where for all choices of hypothesis tests $\bH_1^{i-1} = (H_1, \cdots, H_{i-1})$, we have $\cA_i(\cdot, \bH_1^{i-1})$ has $\beta_i$ - approximate max-information at most $k_i$.  We will define the composed hypothesis test as $\cA: \cX^n \to \cH_m$ where we define $\cA(\bbx)$ in the following way
\begin{itemize}
\item Let $h_1 = \cA_1(\bbx)$
\item For $i = 2, \cdots, m$: set $h_i = \cA_i(\bbx, \bh_1^{i-1})$
\item Return $h_m$.  
\end{itemize}

We then know that $\cA$ has $\sum_{i=1}^m\beta_i$-approximate max-information at most $\sum_{i=1}^m k_i$.  Further, for $H = \cA(\bX)$ we have
$$
\prob{H(\bX) \leq \alpha} \leq  \alpha \cdot 2^{\sum_{i=1}^m k_i}  + \sum_{i=1}^m \beta_i.
$$
\fi




==> rw.tex <==
\section{Related Work}


% Adapative Data Analysis
This paper falls into a recent line of research in adaptive data analysis that originated with Dwork et al. \cite{DFHPRR15STOC}.  They consider the problem of answering an adaptively chosen sequence of statistical queries on a dataset drawn from an unknown distribution, with guarantees that the provided answers approximate the true answers to the queries when evaluated on the underlying distribution. Their main result is that although naive query answering strategies fail, \emph{differential privacy} (an algorithmic stability guarantee introduced by \cite{DMNS06}) of the query answering algorithm, together with \emph{accuracy with respect to the sample} gives a sufficient condition to guarantee that answers generalize to be accurate with respect to the underlying distribution. In particular, leveraging existing algorithms for privately answering large numbers of queries, this yields algorithms capable of answering nearly exponentially many (in the size of the dataset) adaptively chosen queries with non-trivial accuracy. The connection between differential privacy and generalization was extended and strengthened by Bassily et al. \cite{BNSSSU15} who both extend the connection between privacy and generalization beyond statistical queries (to arbitrary low sensitivity queries, and in particular to optimization queries), and give an \emph{optimal} quantitative dependence between the privacy parameters and the resulting generalization guarantees.  Both \cite{BNSSSU15} and \cite{RZ15} extend the connection between algorithmic stability and generalization to weaker notions of algorithmic stability, like total variation distance and KL-divergence, at the necessary cost of relaxing high probability generalization guarantees to guarantees that hold only in expectation. Steinke and Ullman \cite{SU15} (building on the work of Hardt and Ullman \cite{HU14}) show computational hardness results for algorithms capable of accurately answering more than quadratically many arbitrary adaptively chosen queries. 


% Max Information
Dwork et al. \cite{DFHPRR15NIPS} showed that in addition to differential privacy, providing short description length outputs is also a sufficient condition on an algorithm in order to guarantee that its output generalizes to the distribution from which the data was drawn, with high probability. They introduce the notion of \emph{max-information} (a worst case variant of KL-divergence) which (when bounded) guarantees high probability generalization, satisfies strong adaptive composition properties, and which they show to be bounded by algorithms which satisfy both bounded description length, and \emph{pure} differential privacy. This unifies the generalization guarantees known to follow from pure differential privacy and from description length bounds, and allows subroutines satisfying each condition to be composed together. One gap left open by \cite{DFHPRR15NIPS} is that they do not show that algorithms satisfying the constraint of \emph{approximate} differential privacy have bounded max information, which is important because significantly stronger generalization guarantees are known for algorithms satisfying approximate differential privacy \cite{DFHPRR15STOC,BNSSSU15}. This is the question that we address in our work. 

% Mutual Information
\asnote{Add references to Zou and Russo as well as Wang, Lei, Feinberg}
Another line of work \cite{RZ15,WLF16} deals with adaptively chosen queries that are \emph{(sub)-gaussian} and obtains bounds on the maximum expected absolute error in terms of the mutual information between the query answers and the underlying dataset.  Although they do not obtain high probability bounds, \cite{RZ15} gives an application of their results to adaptive feature selection.  
%From \cite{De12}, the mutual information for $(\epsilon,\delta)$-differentially private mechanisms can be large (even for exponentially small $\delta$), the bounds from \cite{RZ15, WLF16} are not strong enough for our setting.  


% Proof Techniques
\asnote{Compare to reults of McGregor et al. and De on the information content of differentially private algorithms.}
To prove our max-information bound for $(\epsilon,\delta)$-differentially private mechanisms, we modify the proof of \emph{adaptive composition} from \cite{DRV10}, where they transform the privacy loss as a sum of martingale differences and apply Azuma's inequality.  To prove how naive composition can lead to overfitting, we apply some useful techniques from \cite{De12} and \cite{MMPRTV11}.  \rynote{elaborate}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:

